There Will Be Spam: Characterizing State-Invariant Transactions and Speculative MEV

Blockchains rely on transparency and immutability to ensure trust, but these guarantees come at the cost of an ever-growing ledger that increasingly threatens decentralization by making it more expensive to store and maintain the full transaction history. In this work, we introduce state-invariant transactions, defined as transactions whose inclusion or removal does not affect the resulting blockchain state beyond transaction fees. We argue that these transactions constitute a form of on-chain spam because they consume execution, bandwidth, storage, and blockspace without contributing to the final ledger state. We present the first large-scale measurement of state-invariant transactions across Ethereum, Optimism, and Base, identifying nearly 1.4 billion such transactions. While only 2.6% of Ethereum transactions are state-invariant, they account for 24% of transactions on Optimism and 37% on Base, representing a significant source of unnecessary resource consumption on Layer-2 blockchains. We show that speculative Maximal Extractable Value (MEV) is the dominant source of state-invariant transactions on Optimism and Base, accounting for 57% and 68%, respectively, but is not the only source as previously assumed. Moreover, despite its popularity, speculative MEV is not the most profitable strategy once the costs of state-invariant transactions are considered. Beyond MEV, we identify substantial malicious activity, with address poisoning campaigns accounting for 53% of non-reverted state-invariant transactions on Ethereum. Our findings suggest that mitigating state-invariant transactions could substantially reduce blockchain resource consumption and transaction costs while limiting phishing campaigns and other forms of blockchain abuse.

==> preamble.tex <==
%! TEX root = ../main.tex
% \RequirePackage{amsmath}
% \documentclass[runningheads]{llncs}
% \let\proof\relax\let\endproof\relax % To use amsthm together with llncs

% \documentclass{article}
% \usepackage[letterpaper]{geometry}
% \pagenumbering{gobble}
% \input{preamble}
% \begin{document}
% \author{
% Aviv Yaish$^{1,3}$ \and
% Benjamin Livshits$^{2,3}$
% }
% \date{
% $^1$The Hebrew University of Jerusalem, Israel \\
% $^2$Imperial College London, UK \\
% $^3$Matter Labs
% }

%% Ifs
\newif\iflong   % For longer versions of the paper
\newif\ifmorecites
\newif\ifanonymous
\newif\ifcomments   % For our comments

\anonymousfalse
\commentstrue
% \anonymoustrue
% \commentsfalse

% %% Try to reduce the number of lines
% \everypar{\looseness=-1 }   % Can be reduced (need a space to terminate the number, otherwise if the paragraph started with 3 \looseness would be set to -13)
% \linepenalty=8000           % Can be increased
% \raggedbottom               % This can be used if we don't want text to fill the entire vertical space of the page, and this can also save space in the beginning of the document

%% Packages
\usepackage[T1]{fontenc}    % Forces T1 fonts, which are supposed to be nicer than the standard ones
\usepackage[english]{babel} % Allows to use special characters, translates some elements within the document, automatically activates the appropriate hyphenation rules for the language you choose. 
\usepackage{mathtools}      % For creating paired delimiters, such as ceil
% \usepackage[english]{babel} % Allows to use special characters, translates some elements within the document, automatically activates the appropriate hyphenation rules for the language you choose. 
% \usepackage{subcaption}     % Allows putting figures side-by-side or one-on-top-of-the-other
% \usepackage[ruled,linesnumbered]{algorithm2e} % For algorithms
\usepackage{enumitem}       % For creating nice enumerated environments
\usepackage{graphicx}       % For specifying image location
\graphicspath{ {./images/} }
\usepackage{booktabs}       % Pretty tables
\usepackage{array,multirow} % For multiple rows/columns in tables
\usepackage{tabularx}       % Can specify column length in tables
% \usepackage{amsthm}         % To manually create theorem environments
\usepackage{amsfonts}
\usepackage{thmtools,thm-restate}   % To restate theorems (define them in one place, and then restate them someplace else)
\usepackage{xcolor}         % Can set nice colors for hyperlinks
\usepackage{hyperref} % For linking to websites
\hypersetup{                % Remove boxes from links, color them instead
    colorlinks,
    linkcolor={red!50!black},
    citecolor={blue!50!black},
    urlcolor={blue!80!black}
}
% \usepackage{minted} % For embedding code, e.g. python
% \usemintedstyle{colorful} % See available styles here https://www.overleaf.com/learn/latex/Code_Highlighting_with_minted#Reference_guide
\usepackage{csquotes}       % Nicer quotes, uses special commands, see https://tex.stackexchange.com/a/39302
\usepackage[capitalise]{cleveref}       % Automatically adds "Section", "Table", etc' to references. Should be imported after all packages
% \usepackage{subfiles} % For working with multiple content .tex files, allows each file to be compiled separately, best loaded last in the preamble

%% Comments
\setlength {\marginparwidth }{2cm}  % Increase margins for notes
\usepackage[colorinlistoftodos,prependcaption,textsize=tiny,textwidth=\marginparwidth]{todonotes}
\newcommand{\aviv}[1]{\ifcomments {\todo[color=blue!40,inline]{Aviv: #1}} \fi}
\newcommand{\ben}[1]{\ifcomments {\todo[color=red!40,inline]{Ben: #1}} \fi}

%% Theorems
% \newtheorem{definition}{Definition}
% \newtheorem{theorem}{Theorem}
% \newtheorem{claim}{Claim}
% \newtheorem{lemma}{Lemma}
% \newtheorem{corollary}{Corollary}
% \newtheorem{example}{Example}
% \newtheorem*{example*}{Example}
% \newtheorem{casestudy}{Case Study}
% \newtheorem*{casestudy*}{Case Study}
% \newtheorem*{discussion*}{Discussion}
% \newtheorem{remark}{Remark}

%% Define reference labels, for cleveref
\crefname{definition}{Definition}{Definitions}
\crefname{theorem}{Theorem}{Theorems}
\crefname{claim}{Claim}{Claims}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{example}{Example}{Examples}
\crefname{remark}{Remark}{Remarks}
\crefname{code}{Code}{Code}

%% Math operators
\DeclareMathOperator*{\argmax}{arg\,\max}
\DeclareMathOperator*{\argmin}{arg\,\min}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}
\newcommand{\expectation}[1]{\mathrm{E} \left[ {#1} \right]}
\newcommand{\variance}[1]{\mathrm{Var} \left[ {#1} \right]}
\newcommand{\define}{\stackrel{\mathclap{\tiny\mbox{def}}}{=}}

%% Glossary (Acronyms and Notations)
% For easily creating a table of glossaries and acronyms. "glossaries-extra" has nice built-in support for symbols, while "glossaries" doesn't
% If entries are not sorted, nogroupskip prevents adding random whitespace between them
% Using '\gls[hyper=true]{bitcoin}' will cancel the automatic hyperlink
\usepackage[symbols,acronym,nonumberlist,nogroupskip,stylemods={mcols,longbooktabs},section=subsection]{glossaries-extra}
% \makenoidxglossaries

% Acronyms
\setabbreviationstyle[acronym]{long-short}  % Will show the first acronym like so: <long-version> (<short-version>)
\glssetcategoryattribute{acronym}{nohyper}{true} % Disable 

\newacronym[longplural={Markov decision processes}]{MDP}{MDP}{Markov decision process}
\newacronym{AI}{AI}{artificial intelligence}
\newacronym{AMM}{AMM}{automated market maker}
\newacronym{APY}{APY}{annual percentage yield}
\newacronym{APR}{APR}{per block interest rate (non compounding)}
\newacronym{ASIC}{ASIC}{application specific integrated circuit}
\newacronym{CDF}{CDF}{cumulative density function}
\newacronym{CPU}{CPU}{central processing unit}
\newacronym{DAA}{DAA}{difficulty-adjustment algorithm}
\newacronym{DQL}{DQL}{deep-Q-learning}
\newacronym{DeFi}{DeFi}{decentralized finance}
\newacronym{EIP}{EIP}{Ethereum improvement proposal}
\newacronym{ERC}{ERC}{Ethereum request for comments}
\newacronym{EVM}{EVM}{Ethereum virtual machine}
\newacronym{HUJI}{HUJI}{Hebrew University of Jerusalem, Israel}
\newacronym{LP}{LP}{liquidity provider}
\newacronym{LT}{LT}{liquidity taker}
\newacronym{MEV}{MEV}{miner-extractable value}
\newacronym{BEV}{BEV}{blockchain-extractable value}
\newacronym{ML}{ML}{machine learning}
\newacronym{OO}{OO}{order optimization}
\newacronym{PDF}{PDF}{probability density function}
\newacronym{PID}{PID}{proportional integral derivative}
\newacronym{PoS}{PoS}{proof-of-stake}
\newacronym{PoW}{PoW}{proof-of-work}
\newacronym{RAM}{RAM}{random-access memory}
\newacronym{RL}{RL}{reinforcement learning}
\newacronym{RPC}{RPC}{remote procedure call}
\newacronym{SSD}{SSD}{solid state drive}
\newacronym{TD}{TD}{total difficulty}
\newacronym{URL}{URL}{uniform resource locator}
\newacronym{USD}{USD}{United States Dollar}
\newacronym{WETH}{WETH}{Wrapped Ethereum}
\newacronym{WBTC}{WBTC}{Wrapped Bitcoin}
\newacronym{YAML}{YAML}{YAML Ain't Markup Language}
\newacronym{block-DAG}{block-DAG}{block directed-acyclic-graph}
\newacronym{geth}{geth}{Go Ethereum}
\newacronym{p2p}{p2p}{peer to peer}
\newacronym{FaaS}{FaaS}{front-running-as-a-service}
\newacronym{FSL}{FSL}{fixed spread liquidation}
\newacronym{DEX}{DEX}{decentralized exchange}
\newacronym{TVL}{TVL}{total value locked}
\newacronym{CPAMM}{CPAMM}{constant product automated market maker}
\newacronym{CFMM}{CFMM}{constant function market maker}
\newacronym{TFM}{TFM}{transaction fee mechanism}
\newacronym{IC}{IC}{incentive compatible}
\newacronym{FN}{FN}{false name}
\newacronym{MIC}{MIC}{miner incentive compatible}
\newacronym{wrt}{w.r.t.}{with regards to}
\newacronym{QoS}{QoS}{Quality-of-Service}
\newacronym{NFT}{NFT}{non-fungible token}
\newacronym{ENS}{ENS}{Ethereum Name Service}
\newacronym{L1}{L1}{layer-1 blockchain}
\newacronym{L2}{L2}{layer-2 blockchain}
\newacronym{ABI}{ABI}{Application Binary Interface}



%% Paper notations
\glsxtrnewsymbol[description={
    A single block.
}]{block}{
    \ensuremath{b}
}
\newcommand{\block}{{\gls[hyper=false]{block}}}

\setcounter{topnumber}{4}
\setcounter{bottomnumber}{4}
\setcounter{totalnumber}{8}


